A Benchmark on Directed Graph Representation Learning in Hardware Designs

To keep pace with the rapid advancements in design complexity within modern computing systems, directed graph representation learning (DGRL) has become crucial, particularly for encoding circuit netlists, computational graphs, and developing surrogate models for hardware performance prediction. However, DGRL remains relatively unexplored, especially in the hardware domain, mainly due to the lack of comprehensive and user-friendly benchmarks. This study presents a novel benchmark comprising five hardware design datasets and 13 prediction tasks spanning various levels of circuit abstraction. We evaluate 21 DGRL models, employing diverse graph neural networks and graph transformers (GTs) as backbones, enhanced by positional encodings (PEs) tailored for directed graphs. Our results highlight that bidirected (BI) message passing neural networks (MPNNs) and robust PEs significantly enhance model performance. Notably, the top-performing models include PE-enhanced GTs interleaved with BI-MPNN layers and BI-Graph Isomorphism Network, both surpassing baselines across the 13 tasks. Additionally, our investigation into out-of-distribution (OOD) performance emphasizes the urgent need to improve OOD generalization in DGRL models. This benchmark, implemented with a modular codebase, streamlines the evaluation of DGRL models for both hardware and ML practitioners

==> arxiv/008-check_list.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{See Section~\ref{app:dataset_selection_detail}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Section~\ref{app:dataset_selection_detail}}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> arxiv/old_expe.tex <==
\section{Experiments}
We explore the combinations within the design space of directed graph encoders. The experiment results across all the five datasets on both in-distribution (ID) and out-of-distribution (OOD) testing data for thirteen tasks with thirteen evaluation metrics are reported in Appendix.~\ref{app:exp_main_result} in detail.
Based on the results, we first discuss \pan{compare} the design of each component (the message passing strategy, the selection of the GNN backbone, and structural feature augmentation by positional encoding), to obtain insights on how different choices on each part may impact the expressiveness, scalability, and generalization \pan{do you have literally expressiveness scalability comparison? checking function approximation and checking scaling?} of the GNN encoder. Then we summarize the results, identify a recipe of GNN encoder design for directed graph representation learning with applications in circuits. 

\subsection{Insights to share on the design of Key Components}

\pan{Let people know that we have for each task, each combination of model design, a specific evaluation score. Here is just ranking for comparison purpose.}

\subsubsection{GNN Backbone Selection \pan{GPS use native node-PE} \pan{Bi-direction, unify table 6 and table 7. Add more directed graph encoders.} }
\input{neurips_data_2024/tables/summary/backbone_selection}
We compile the average rankings of GNN backbones on all tasks and corresponding evaluation metrics for both in-distribution (ID) and out-of-distribution (OOD) testing data across all the datasets. The results are presented in Table.~\ref{tab:exp_gnn_backbone_selection} \pan{why EPE not for SR, TIME CG? Is PE/EPE used in GCN, GAT, GIN? if no, the comparison is unfair} \pan{The better way is to give a big table and compare the scores therein. Or compare the best scores (with PE) across different baselines  or compare the scores across different baseines with the same PE technique}, where the detailed methodology for calculating the rankings is described in Equation.~\ref{equ:gnn_backbone_ranking_calculation_expression} in Appendix.~\ref{app:gnn_backbone_ranking_expression}.
All models employ the basic `plane' (-) message passing strategy. Except for GPS, none includes PE. Due to the necessity of incorporating PE with transformers, GPS adopts EPE. We observe that GPS perform the best on both in-distribution (ID) and out-of-distribution (OOD) tests on smaller circuit datasets (HLS and AMP), demonstrating excellent expressiveness \pan{we cannot use expressiveness here...} and good generalization capabilities \pan{We can only say in-distribution or out-of-distribution}. However, GPS is unable to operate on larger graphs with up to tens of thousands of nodes due to scalability limitation, whereas other backbones do not face such issues. Among the other backbones, MSGNN demonstrates superior performance on large graph ID testing data where the training and test graph structures are very similar, aligning with ~\cite{he2022msgnn} that MSGNN performs the best on directed finance/social networks where training and testing may take on same graph structures, while in OOD tests, MSGNN is surpassed by GIN(E). Overall, considering both ID and OOD test data, GIN(E) ranks the highest. \textit{In conclusion, GPS is well-suited for small (around one hundred nodes) directed circuit graphs. For more general scenarios requiring a balance of scalability, expressive power, and generalization, we recommend using GIN(E) as the backbone.}

Note that in Appendix.~\ref{app:gps_p} we use TIME dataset to illustrate the performance of GPS-P, which employs efficient transformer layer (Performer). While scalability is improved, its ID performance is not so good as GINE which is solely based on message passing. In OOD tests, GPS-P only achieves performance comparable to GINE.

\subsubsection{Message Passing Strategy}
\input{neurips_data_2024/tables/summary/bidi}
We report the average rankings of message passing strategies on three backbones: GCN, GIN(E), and GAT on both ID and OOD test sets. The method for calculating the rankings is detailed in Equation.~\ref{equ:message_passing_ranking_calculation_expression} in Appendix.~\ref{app:message_passing_expression}. Results confirm that `bidirected' (BI) message passing method outperforms the other two approaches on in-distribution (ID) circuit graphs, consistent with previous findings on other type of directed graphs~\cite{wen2020neural, jaume2019edgnn}. The superior performance is attributed to the enhanced expressive power from distinct NN parameters along two edge directions. Furthermore, we find that (BI) still performs the best on OOD circuit graphs, indicating that empirically its enhanced expressiveness does not affect generalization. As to (DI) and (-), there is no clear evidence indicating a definitive advantage between them. \textit{In conclusion, we recommend using (BI) strategy for directed graph encoders.} \pan{We should compare using two direction edges but with the same parameters, perhaps using edge features to distinguish}

\subsubsection{Structural Feature Augmentation by Positional Encoding} \pan{require + GPS}
Next, we discuss the impact of incorporating PE on encoders. We report the performance of NNs under three conditions: without PE, with `node PE' (NPE), and with `edge PE' (EPE). The detailed results are shown in Appendix.~\ref{app:result_npe_epe}. We summarize the average rankings of different PE on GIN(E) and BI-GIN(E), as shown in Table.~\ref{tab:ne} \pan{where are other backbones, especially GPS?}. The relevant calculation is detailed in Equation.~\ref{equ:structural_feature_augmentation_ranking_calculation_expression} in Appendix.~\ref{app:structural_feature_augmentation_ranking_expression}. \hy{quantity result to add?}
\input{neurips_data_2024/tables/summary/ne}

Results show that EPE significantly enhances the encoder's performance on both ID and OOD testing data. However, improvements are not observed with NPE. On directed circuit graphs, naively concatenating eigenvectors from MagLap decomposition to nodes does not improve ID performance and even degrade OOD performance, because NPE is unstable and fails to address the non-uniqueness of MagLap decomposition. Conversely, incorporating PE using stable methods~\cite{huang2023stability} boosts performance on both ID and OOD datasets by providing a more robust integration of extra structural features. \textit{In conclusion, we recommend adopting SPE for structural feature augmentation.}

Note that in this benchmark, we select two potential values \( q = 0 \) \pan{why $q=0$? does this just go back to symmetric lap?} and \( q = 0.1 \) for MagLap \pan{in this case, the parameter spaces sound too small...}. Adjusting \( q \) on a specific task may further enhance the encoder's performance. Using GPS+EPE on the AMP datas as an example, we conduct a grid search for \( q \) and find that \( q = 0.03 \) yields the best performance, as shown in Table.~\ref{tab:amp_gain_qvalue} in Appendix.~\ref{app:q_value}.


\subsection{Summary: Recipe for Directed Graph Learning}

\input{neurips_data_2024/tables/summary/compare_baselines}

\input{neurips_data_2024/tables/summary/id_ood}
After discussing the different choices within the design space for each component, we summarize the overall performance in Table.~\ref{tab:id_ood} \pan{I still think we should give a full table with minimum-necessary summary.}, where we display the score measuring `on average, how many datasets that the method ranks the first or within the top three'. The score calculation is detailed in Equation.~\ref{equ:main_result_calculation_expression} \pan{as this is too abstract, I think the way to compute this score should be in the main text} in Appendix.~\ref{app:exp_main_result}. BI-GINE+EPE based on empirical insights from the previous sections, is easily to deploy across all the circuit scales, achieves first place in about half of the datasets and ranks within the top three in almost all datasets for both ID and OOD data. Ensuring scalability, `BI-GINE+EP achieves the best in both expressiveness power and generalization.

\hy{Further verification on Google TPUgraph competition dataset}
\pan{for google TPU, at least we should try a few benchmarks. }

\textbf{Recipe for directed graph learning:} \textit{ From results on circuit data, we propose a design recipe for encoders on directed graphs: `BI-GNN+EPE'. We recommend using a `bidirected' message passing strategy and incorporating stably processed PE as structural feature augmentation.}

We further compare `BI-GNN+EPE' with the approaches designed specifically for each dataset as reported in their original papers. The results are show in Table.~\ref{tab:compare_baselines} \pan{this should be emphasized a lot in the intro}. Since the original papers do not consider OOD issues, our comparison focus on ID performance. BI-GINE+EPE achieves results comparable to, or even better than, the methods proposed in the original papers. It is important to note that methods specifically designed for certain circuits may incorporate domain-specific expert knowledge and additional data processing. For example, CKTGNN~\cite{dong2023cktgnn} in the AMP dataset modifies the structure of circuits into DAGs and employs an asynchronized message passing strategy; In the TIME dataset, `timer-GNN'~\cite{guo2022timing} is tailored to mimic the transmission rules of clock signals and designs a non-linear delay model (NLDM) along with a `cell library'. Additionally, some methods may not be based on data-driven approaches: in the CG dataset, `nn-meter'~\cite{zhang2021nn} utilizes a kernel-based encoder and manually crafts input feature based on expert knowledge. These underscore the strong performance of the general recipe, BI-GINE+EPE, and also highlight the promising potential of further enhancing our model by incorporating domain-specific knowledge.















==> arxiv/old_intro.tex <==
\textbf{motivation}
1. The definition, wide usage of EDA. ML encoders have been widely used in EDA design to predict xxx.

2. Among the problems, many could be represented into directed graphs, and 

[ML helps EDA]GNNs are naturally considered a proper method to encode the directed graph data and many EDA-domain works train GNN as encoders to achieve very promising results. 

[EDA helps ML] The directed graph representation in EDA domain often includes logic reasoning or flow control on the graphs, which is less common in other domain whose data could be represented as directed graphs (e.g. social network, finance network). Therefore, EDA tasks actually servers as a good real-world application to showcase and valid the ML theoretic progress.


3. Current graph ML for EDA papers takes the advantage of strong domain knowledge into the pipeline (data-processing, GNN structure design), which may use some handcraft data-processing/features to achieve. We want to see if some latest new techniques in graph ML domain could likely provide a general recipe for automatics model design that is even likely to further improve the performance.

4. To design a general graph model for EDA, we pose several questions: 1) how to control the message passing in circuits (directed graphs) directed / undirected message passing? 2) does recent progress in positional encoding (PE) work in circuit tasks? 3) Would the model preserve performance in OOD tasks?

\textbf{comparison} Compared with existing benchmark papers:
1. PyGSD~\cite{he2022pytorch}: this paper focuses on directed/signed networks (single graph, node level/link prediction task, which is different from computational-flow like circuits). Datasets are for social network or finance flow map. We also include the best method MSGNN~\cite{he2022msgnn} as a baseline to benchmark form this paper. application. method: logical reasoning. graph filtering, spectral - logical, PE. task: node - graph.

2. GPS~\cite{rampavsek2022recipe}. The PyG implementation only includes NPE, no EPE. we take it as an important baseline. (transformer not time-efficient in large graphs). application, methodology, task.
undirected graph. 

3. ~\cite{bai2023towards} is HLS benchmark, with pre-trained LLM.


5. contributions:

$\bullet$ We benchmarks the designing strategies on designing GNN encoders in circuit tasks to answer the questions above and obtain the insights of designing GNN encoders for EDA encoder:

[To tell the EDA people how to design]bi>plain>di, adding edge-level magnetic laplacian PE is better

[To tell the ML people] SPE is indeed useful in EDA domain applications, which includes logic reasoning and flow control tasks.

[OOD performance] As to OOD cases, in amplified graph structure / only local information is required cases, GNNs could maintain generalization ability, but in the scenario where limited structures are provided and require global reasoning, it's still very challenging. 



$\bullet$ We propose a recipe to build a general GNN encoder baseline for future research. We are the first to design bi-directional different weight message passing + stable edge positional encoding. The baseline is without in-depth application specific knowledge, but achieves better results than the designed methods in each task in ID and OOD tasks. 


$\bullet$ We open-source the code, form a framework, easy to plug-in any other EDA problems that could be formulated as directed graphs, to provide the EDA domain an easier toolbox to tune their model and get the results.

==> arxiv/old_method.tex <==
\section{Benchmark Design}
%\pan{Introduce why you choose these backbones, why they are representative, why consider PE, why stable PE, why consider transformer, }

\subsection{Problem Formulation and Encoder Design Space}

\begin{figure}[h] % [H] 选项确保图片和表格在当前位置显示
    \centering
    \begin{minipage}{0.55\textwidth} % 图片的宽度
        \centering
        \includegraphics[width=\linewidth]{neurips_data_2024/figures/combination_method.pdf} % 替换为你的图片文件名
        \caption{The benchmark considers 20 combinations of message passing, MPNN layers, global attention and PE incorporation in total, covering 10 existing methods from graph ML community and helping discover 2 novel top-performing models (see the right Table).}
    \end{minipage}
    \hfill % 在两个minipage之间插入水平间距
    \begin{minipage}{0.43\textwidth} % 表格的宽度
        \centering
        \resizebox{\textwidth}{!}{\begin{tabular}{@{}ccc@{}}
\toprule
Method & type & \begin{tabular}[c]{@{}c@{}}layer-wise\\ complexity\end{tabular} \\ \midrule
GCN~\cite{kipf2016semi} & spectral & $O(|E|)$ \\
MagNet~\cite{zhang2021magnet} & spectral & $O(|E|)$ \\
DGCN~\cite{tong2020directed} & spectral & $O(|E|)$ \\
DiGCN~\cite{tong2020digraph} & spectral & $O(|E|)$ \\ \midrule
GAT~\cite{velivckovic2017graph} & spatial & $O(|E|)$ \\
GIN(E)~\cite{xu2018powerful} & spatial & $O(|E|)$ \\
EDGNN~\cite{jaume2019edgnn} & spatial & $O(|E|)$ \\ \midrule
GPS-T~\cite{rampavsek2022recipe} & spatial+transformer & $O(|V|^2 + |E|)$ \\
GPS-P~\cite{choromanski2020rethinking} & spatial+transformer & $O(|V|+|E|)$ \\
TmD~\cite{geisler2023transformers} & transformer & $O(|V|^2)$ \\ \midrule
BI-GIN(E)+EPE & spatial & $O(|E|)$ \\
BI-GPS+EPE & spatial+transformer & $O(|V|^2 + |E|)$ \\ \bottomrule
\end{tabular}}
\vspace{-0.cm}
\caption{Existing and proposed methods.}
    \end{minipage}
\end{figure}


Let $G(V, E)$ denote a directed graph with $V$ representing the node set and $E$ the edge set. `Directed' refers that $(u,v) \in E$ does not imply $(v,u) \in E$. We call $u$ successor of $v$ if $(v,u) \in E$ and predecessor if $(u,v) \in E$.
Let $\mathcal{Y}$ be the output space, 
%$l: \mathcal{Y} \times \mathcal{Y} \rightarrow \mathbb{R}$ be the evaluation loss. 
the objective is to identify a graph encoder designing strategy $f^*$ from design space $\mathcal{F}$ that after training 
%on distribution $\mathbb{P}_{\mathcal{S}}(G,y)$ 
achieves low loss on both in-distribution test data and the test data that exhibit distribution shifts. %$\mathbb{P}_{\mathcal{T}}(G, y) \neq \mathbb{P}_{\mathcal{S}}(G, y)$.
Design space $\mathcal{F}$ can be broken down into three parts: the selection of GNN backbones, the strategy of message passing and the incorporation of PE. 
Note that we do not consider the backbones~\cite{luo2024transformers, rey2024convolutional} or message passing strategies~\cite{zhang2019d, thost2021directed} that are only applicable to directed acyclic graphs (DAGs)~\cite{digitale2022tutorial}. Our benchmark aims to explore general directed graphs and thus includes circuit data not limited to DAGs.
The $k$-th layer of encoder could be represented as: \pan{slightly confused about the following Eq.1. Can it incorporate GPS?}
\vspace{-0.2cm}
\begin{equation}
\label{equ:design_space}
\begin{aligned}
    & f^{(k)}(\cdot; \theta) \ : \ \  \bm{x}_i^{(k)} = \gamma^{(k)} \left( \Psi_i^{(k-1)},  \bigoplus_{j \in \overset{\longrightarrow}{\mathcal{N}(i)}} \, [\Phi^{(k)}_{j,i,\rightarrow}], \bigoplus_{j \in \overset{\longleftarrow}{\mathcal{N}(i)}} \, [\Phi^{(k)}_{j,i,\leftarrow} ]; \theta_{\gamma} \right),  \\
      \text{where} & \ \ \Phi^{(k)}_{j,i,\rightarrow} = \phi^{(k)}(\Psi^{(k-1)}_i, \Psi_j^{(k-1)}, \Xi^{(k-1)}_{j,i}; \overset{\rightarrow}{\theta_{\phi}}), \\
      & \ \ \Phi^{(k)}_{j,i,\leftarrow} = \phi^{(k)}(\Psi^{(k-1)}_i, \Psi_j^{(k-1)}, \Xi^{(k-1)}_{j,i}; \overset{\leftarrow}{\theta_{\phi}}),
     \\ \ \ & \Psi^{(k-1)}_i = \psi^{(k-1)}(\bm{x}_i^{(k-1)}, \bm{z}_i; \theta_{\psi}), \ \ \Xi_{j,i}^{(k-1)} = \xi^{(k-1)}(\bm{e}_{j,i}^{(k-1)}, \bm{z}_{j}, \bm{z}_{i}; \theta_{\xi}), 
\end{aligned}
\end{equation}
\begin{wraptable}{r}{0.45 \textwidth}
\vspace{-0.35cm}
\resizebox{0.45 \textwidth}{!}{\begin{tabular}{@{}cc@{}}
\toprule
design space                                                               & encoder function/variable \\ \midrule
backbone                                                                   & $\gamma(\cdot; \theta_{\gamma})$,  $\phi(\cdot; \theta_{\phi})$                  \\ \midrule
message passing                                                            &  $\{ \overset{\rightarrow}{\theta_{\phi}},\overset{\leftarrow}{\theta_{\phi}}\} $               \\ \midrule
\begin{tabular}[c]{@{}c@{}}structural feature \\ augmentation\end{tabular} &   $\bm{z}$, $\psi(\cdot; \theta_{\psi})$, $\xi(\cdot; \theta_{\xi})$                 \\ \bottomrule
\end{tabular}}
\vspace{-0.2cm}
\caption{Design space \& functions/variables. \pan{avoid using structral features; use PEs as you only use PEs. Also $z$ does not mention.} }
\vspace{-0.45cm}
\label{tab:design_space}
\end{wraptable}
 $\bm{x}_i^{(k)}$, $\bm{e}_{j,i}^{(k)}$ denotes the node/edge feature at $k$-th layer, $\bm{z}$ could be PE, $\Psi_i^{(k)}, \Xi_i^{(k)}$ denotes the node/edge representation enhanced with PE if applied; $\gamma(\cdot; \theta_{\gamma})$, $\phi(\cdot; \theta_{\phi})$ are parameterized functions determined by GNN backbones; $\oplus$ denotes a permutation invariant aggregation function, $\overset{\longrightarrow}{\mathcal{N}(i)}, \overset{\longleftarrow}{\mathcal{N}(i)}$ denotes the set of one-hop successors and predecessors of node $i$; $\overset{\rightarrow}{\theta_{\phi}}, \overset{\leftarrow}{\theta_{\phi}}$ are the parameters that control message passing on forward and reverse directions of edges on the directed graph; $\psi(\cdot; \theta_{\psi}), \xi(\cdot; \theta_{\xi})$ are functions that incorporate PE into node/edge features. We outline the three parts and the corresponding functions/variables that they determine in Table.~\ref{tab:design_space}. Next, we provide detailed description of the benchmarking design space for each part.
\subsection{GNN Backbone Selection \pan{4.3 merged into 4.2 (please smooth the discussion. Check my comments in the end of 4.2).  4.4 can be separated. }}
\begin{wraptable}{r}{0.5 \textwidth}
\vspace{-0.4cm}
\renewcommand{\arraystretch}{1.2}
\resizebox{0.5 \textwidth}{!}{\begin{tabular}{ccc}
\hline
 & spectral/spatial & \begin{tabular}[c]{@{}c@{}}layer-wise\\ complexity\end{tabular} \\ \hline
GCN~\cite{kipf2016semi} & spectral & $O(|E|)$ \\
GAT~\cite{velivckovic2017graph} & spatial & $O(|E|)$ \\
GIN~\cite{xu2018powerful} & spatial & $O(|E|)$ \\
GPS-T~\cite{rampavsek2022recipe} & spatial+transformer & $O(|V|^2 + |E|)$ \\
GPS-P~\cite{choromanski2020rethinking} & spatial+transformer & $O(|V|+|E|)$ \\ \hline
MagNet~\cite{zhang2021magnet} & spectral & $O(|E|)$ \\
DGCN~\cite{tong2020directed} & spectral & $O(|E|)$ \\
DiGCN~\cite{tong2020digraph} & spectral & $O(|E|)$ \\ \hline
\end{tabular}}
\vspace{-0.2cm}
\caption{Comparison of the backbones. \pan{do we need to add directed transformer. Or we should explain that GPS-T is directed transformer}}
\vspace{-0.3cm}
\label{tab:gnn_backbone}
\end{wraptable}
The selection of backbone determines how edge and node features are encoded, aggregated, or globally reasoned, which are shown in Table.~\ref{tab:gnn_backbone}. For backbones designed for undirected graphs, we start with GCN~\cite{kipf2016semi}, GIN~\cite{xu2018powerful}, and GAT~\cite{velivckovic2017graph} that share similar time complexity and expressiveness. We further explore GPS-T~\cite{rampavsek2022recipe} that integrates GIN layers with transformer layers~\cite{vaswani2017attention} to achieve higher expressive power through global attention reasoning. However, the scalability of GPS is undesirably reduced due to the extensive attention calculations required for node pairs. GPS-P with efficient transformer (performer~\cite{choromanski2020rethinking}) is included in the study as well, yet it performs similarly at best but still much slower than backbones that rely solely on message-passing. High-order GNNs~\cite{maron2019provably, maron2018invariant, morris2019weisfeiler, frasca2022understanding} are not considered, as they require complexity even greater than GPS, making them impractical to run on the scale of real-world circuits. As to methods especially designed for directed graphs, we pick DGCN~\cite{tong2020directed}, DiGCN~\cite{tong2020digraph} and MagNet~\cite{zhang2021magnet}, covering the methods for directed social or financial network representation learning used in PyGSD benchmark~\cite{he2022pytorch} \pan{``covering xxx'' is useless. To emphasize the coverage our benchmark, saying these methods from other benchmarks is a bad evidence. Think about what is a good angle to sell these methods to show our coverage (perhaps, spectral representative? use spectrum of directed lap (defined in 4.4)? )}. Detailed backbone definitions are in Appendix.~\ref{app:gnn_backbone}.\pan{we miss directed transformers. Also, we should merge 4.3 into 4.2, as 4.3 is a pretty common practice in DGRL domain, no need to be highlighted. After merging, BI-GINE, used in previous work, is also naturally mentioned. Currently, we miss the reference and discussion.}
\pan{The novel thing that should be emphasized is GT + MPNN, as we are the first to use it in DGRL. Given this, I am slightly concerned that we did not evaluate pure GTs.}

\subsection{Message Passing Strategy}
\label{sec:message_passing_strategy}
\begin{wraptable}{r}{0.4 \textwidth}
\vspace{-0.4cm}
\resizebox{0.4 \textwidth}{!}{\begin{tabular}{@{}cc@{}}
\toprule
message passing   & description \\ \midrule
`plane' (-)       & $\overset{\rightarrow}{\theta_{\phi}} = \overset{\leftarrow}{\theta_{\phi}} \neq \mathbf{0}$            \\
`directed' (DI)   & $\overset{\rightarrow}{\theta_{\phi}} \neq \mathbf{0},  \overset{\leftarrow}{\theta_{\phi}} = \mathbf{0}$            \\
`bidirected' (BI) & $\overset{\rightarrow}{\theta_{\phi}} \neq \mathbf{0},  \overset{\leftarrow}{\theta_{\phi}} \neq \mathbf{0}, \overset{\rightarrow}{\theta_{\phi}} \neq \overset{\leftarrow}{\theta_{\phi}}$            \\ \bottomrule
\end{tabular}}
\vspace{-0.2cm}
\caption{Message passing strategy.}
\label{tab:message_passing_strategy}
\vspace{-0.3cm}
\end{wraptable}
\pan{As the strategy is commonly known, I suggest to reduce the emphasis of this paragraph.} On directed graphs, message passing strategy could significantly influence the encoder's expressiveness~\cite{rossi2024edge}. We benchmark three strategies as listed in Table.~\ref{tab:message_passing_strategy}. `Plane' (-) treats directed graphs as undirected, using same NN parameters to perform message passing simultaneously along both forward and reverse edge directions. `directed' (DI) strategy only passes message exclusively along the forward edge directions. As to `bidirected'(BI), it performs message passing in both the forward and reverse directions with distinct parameters for each direction. After propagation, node embeddings are obtained by averaging from both directions. Encoders with `bidirected' strategy theoretically obtain better expressive power~\cite{jaume2019edgnn, kollias2022directed, rossi2024edge, wen2020neural}.



%\subsection{Structural Feature Augmentation \hy{yinan please review}}
\subsection{Direction-aware Positional Encodings} \pan{This paragraph. We should not emphasize maglap too much. Instead, we should emphasize maglap and symmetry lap are just how to select $q$. We view it as a hyperparameter. The new things to be emphasized are stable structures as they are useful in our case. One thing unclear is that in GPS, where to use NPE, where to use EPE, in the MPNN layer or transformer layer. please check with Haoyu.}
%Augmenting the input of encoders with extra graph structural features provably enhances expressiveness~\cite{maron2019provably,wang2022equivariant, you2019position}. High-order GNNs~\cite{maron2019provably, maron2018invariant, morris2019weisfeiler} encode high-order structures (e.g. k-node tuples) as extra feature to achieve stronger expressiveness, which always involves high-dimensional tensor computation, making it impractical to implement on real-world circuit scales\yinan{Do we need to mention high-order methods here? I don't think they belong to structural feature augmentation.}. 

It is known that message passing neural networks suffer from limited expressive power~\cite{xu2018powerful, morris2019weisfeiler}, and positional encodings (PE), as vectorized representations of global positional information for nodes, can provably 
alleviate this problem~\cite{lim2022sign}. Similarly for directed graphs, one can expect that direction-aware PE could help boost the expressive power of directed graph encoders. To this end, we adopt Magnetic Laplacian (MagLap) PE, the eigenvectors of MagLap matrix~\cite{geisler2023transformers}. The MagLap matrix $\bm{L}_q$ is a complex Hermitian matrix with a parameter $q\in[0, 1)$ called potential (see definition at~\cite{furutani2020graph}, Eq.(12)), which is treated as  a hyperparameter in our experiments. It is worth noticing that when $q=0$, MagLap $\bm{L}_{q=0}$ degenerates to the standard symmetric Laplacian matrix as a special case. Following~\cite{geisler2023transformers}, we use the smallest $d$ eigenvalues $\lambda_q \in \mathbb{R}^{d}$ and their corresponding eigenvectors $\bm{V}_q \in \mathbb{C}^{|V| \times d}$ from $\bm{L}_q$.

%MagLap matrix is a Hermitian complex matrix defined by $\bm{L}_q = \bm{I} - \bm{D}^{-1/2} \bm{A}_q \bm{D}^{-1/2}$, where $\bm{D}$ is the diagonalized degree matrix counting both in-degree and out-degree, and $\bm{A}_q$ refers to the complex matrix as follows:
%\begin{equation}
%    [\bm{A}_q]_{u,v} = \left\{ \begin{aligned}
%        \exp\{i2\pi q\}&,&\text{if } (u,v)\in \mathcal{E},\\ 
%         \exp\{-i2\pi q\}&,&\text{if } (v,u)\in \mathcal{E},\\ 
%         1 &, & \text{if } (u,v), (v,u)\in\mathcal{E},
%    \end{aligned} \right.
%\end{equation}
%with a parameter $q\in[0, 1)$ called potential. 
%Following~\cite{geisler2023transformers}, we use the smallest $d$ eigenvalues $\lambda_q \in \mathbb{R}^{d}$ and their corresponding eigenvectors $\bm{V}_q \in \mathbb{R}^{|V| \times d}$ from $\bm{L}_q$. Note that when $q=0$, given $\bm{A}$ as $G$'s adjacency matrix, $\bm{A}_q$ degenerates to the symmetric version of adjacency matrix $\bm{A}_q = \bm{A} + \bm{A}^\top$, and the MagLap turns into the standard Laplacian matrix as a special case.

%Another more cost-acceptable way is to add positional encoding (PE) to encode the pair-wise distance information among nodes~\cite{wang2022equivariant, huang2023stability, lim2022sign} as vectorized features. Note that the design and embedding of PE could significantly determine the encoder's stability and generalization ability~\cite{huang2023stability, wang2022equivariant}. We follow~\cite{geisler2023transformers} to use the smallest $d$ eigenvalues $\lambda_q \in \mathbb{R}^{d}$ and their corresponding eigenvectors $\bm{V}_q \in \mathbb{R}^{|V| \times d}$ from the magnetic~\yinan{Magnetic} Laplacian (magLap) matrix $\bm{L}_q$ of the directed graph $G$ to encode the directional distances, where $\bm{L}_q = \bm{I} - \bm{D}^{-1/2} \bm{A}_q \bm{D}^{-1/2}$, $\bm{D}$ is the diagonalized degree matrix counting both in-degree and out-degree, $\bm{A}_q$ refers to the complex matrix:
%\vspace{-0.2cm}
%\begin{equation}
%    [\bm{A}_q]_{u,v} = \left\{ \begin{aligned}
%        \exp\{i2\pi q\}&,&\text{if } (u,v)\in \mathcal{E},\\ 
%         \exp\{-i2\pi q\}&,&\text{if } (v,u)\in \mathcal{E},\\ 
%         1 &, & \text{if } (u,v), (v,u)\in\mathcal{E},
%    \end{aligned} \right.
%\end{equation}
%where $q \in [0, 1)$ denotes the parameter potential. Note that when $q=0$, given $\bm{A}$ as $G$'s adjacency matrix, $\bm{A}_q$ degenerates to the symmetric version of adjacency matrix $\bm{A}_q = \bm{A} + \bm{A}^\top$, and the magLap turns into the standard Laplacian decomposition as a special case.
\begin{table}[h]
%\vspace{-0.3cm}
\captionsetup{font=footnotesize}
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{@{}ccc@{}}
\toprule
              & obtain PE $\bm{z}$            & embed $\psi(\cdot)$/ $\xi(\cdot)$ \\ \midrule
`node PE' (NPE) & $ \bm{z} =  [\text{Re}\{\bm{V}_q\}, \text{Im}\{\bm{V}_q\}]$ &     $ \psi(\cdot) = \text{concact}(\bm{z}, \bm{x})$     \\ 
\multirow{2}{*}{`edge PE' (EPE)}&  $ \bm{z} = \rho(\text{Re}\{\bm{V_q}\text{diag}(\kappa_1(\lambda))\bm{V_q}^{\dagger}\}, ..., \text{Re}\{\bm{V_q}\text{diag}(\kappa_m(\lambda))\bm{V_q}^{\dagger}\},$&   \multirow{2}{*}{$\xi(\cdot) = \text{concact}(\bm{z}, \bm{e})$}       \\ 
 & \hspace{30pt}$\text{Im}\{\bm{V_q}\text{diag}(\kappa_1(\lambda))\bm{V_q}^{\dagger}\}, ..., \text{Im}\{\bm{V_q}\text{diag}(\kappa_m(\lambda))\bm{V_q}^{\dagger}\})$ & \\\bottomrule
\end{tabular}}
\caption{Functions to obtain and embed PE. NPE directly concatenates the eigenvectors to the node features. In contrast, before concatenating PE to the edge features, EPE employs the permutation equivariant functions $ \kappa : \mathbb{R}^{d} \rightarrow \mathbb{R}^d$ w.r.t. eigenvalue permutations and permutation equivariant function $\rho: \mathbb{R}^{|V|\times |V| \times 2m} \rightarrow \mathbb{R}^{|V| \times |V| \times d}$ to stably process the eigenvectors and eigenvalues, respectively.}
\label{tab:node_edge_PE}
\vspace{-0.4cm}
\end{table}

Note that way of using PE could significantly influence the encoder's stability and generalization ability~\cite{huang2023stability, wang2022equivariant}. To use MagLap PE, we mainly use and compare two approaches: 1) \emph{unstable} `node PE' (NPE): node features are initially concatenated with the raw eigenvectors before feeding into any backbone models. NPE enhances expressive power with minimal additional computational cost, yet it suffers from poor stability or generalization~\cite{wang2022equivariant}; 2) \emph{stable} `edge PE' (EPE), which adopts the framework of SPE~\cite{huang2023stability} to obtain stable and expressive PE as a $|V|\times |V|\times d$ tensor. If the following backbone model leverages a message passing modules, the input edge features are initially concatenated with the EPE tensor with corresponding entries of existing edges like in~\cite{wang2022equivariant}. If the backbone model additionally involves transformer modules (e.g., GPS), the EPE tensor is further added to the attention weight as a bias term at each attention layer. The detailed formulas to obtain and embed EPE and NPE are shown in Table.~\ref{tab:node_edge_PE}.

\subsection{Hyer-Parameter Space and Tuning}
For each combination of directed graph encoding methods in this benchmark, we perform automatic hyper-parameter tuning with RAY~\cite{liaw2018tune} adopting Tree-structured Parzen Estimator (TPE)~\cite{watanabe2023tree}. The hyper-parameter space involves batch size, learning rate, number of backbone layers, dropout rate, hidden dimension, and MLP layer configurations. Detailed hyper-parameter space of each backbone is shown in Appendix.~\ref{app:hyper-parameter_space}. We auto-tune the hyper-parameters with seed $123$ with $100$ trial budgets and select the configuration with the best validation performance. Then the selected configuration trains and tests for ten times with seeds $0-9$ to average for the final performance.



\iffalse
\begin{table}[h]
\resizebox{\textwidth}{!}{\begin{tabular}{@{}cclc@{}}
\toprule
 & \multicolumn{2}{c}{name} & description \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}message\\ passing\\ strategy\end{tabular}} & \multicolumn{2}{c}{undirected MP} & \begin{tabular}[c]{@{}c@{}}regard the directed circuit graph as an undirected graph, \\ do message passing with same GNN parameters on both direction\end{tabular} \\ \cmidrule(l){2-4} 
 & \multicolumn{2}{c}{directed MP} & only conduct message passing following the direction of the circuit \\ \cmidrule(l){2-4} 
 & \multicolumn{2}{c}{bidirected MP} & \begin{tabular}[c]{@{}c@{}}adopt different GNN weight on directed circuit graph and aggregate the latent feature\\ many examples on graph ML domain to handle directed graph: examples yinan talked\end{tabular} \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}obtaining\\ PE\end{tabular}} & \multicolumn{2}{c}{q\textgreater{}0} & do MagLap decomposition \\ \cmidrule(l){2-4} 
 & \multicolumn{2}{c}{q=0 (LAP)} & a pecial case when q = 0, turns to be laplacian decomposition \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}handling\\ PE\end{tabular}} & \multicolumn{2}{c}{node PE (NPE)} & concact the PE embedding in node feature, not stable \\ \cmidrule(l){2-4} 
 & \multicolumn{2}{c}{edge PE (EPE)} & equivariant PE into edge feature, more stable (SPE) \\ \bottomrule
\end{tabular}}
\end{table} \fi






==> arxiv/sketch.tex <==
 \section{Sketch}
\hy{$\bullet$ Question 1. What is the motivation of the paper?}

\hy{\textbf{motivation from EDA domain}: ML based encoders for circuits are more and more widely used in EDA + circuit are mostly formed as directed graphs $\rightarrow$ How to design graph encoders for circuit problems?}

\pan{strong logic dependence needs more powerful encoders; faster simulation, surrogate model, from application side}

\nan{fast, accurate, and scalable performance predictions to accelerate design iterations and DSE; efficient fusion of structural and functional information from circuit graphs}

\hy{\textbf{motivation from ML domain}: There remains an open question: directed graph: How to design encoders for directed graphs?}unfinished

%\pan{Advanced ML tool for directed graph representation}

\hy{$\bullet$ Question 2. What is the benefit of the research?}

\hy{[ML helps EDA] The latest tech (PE) and design strategies for GNNs may help provide a recipe to design circuit encoders.} \pan{more expressiveness not just PE. Using PE ---structure feature augmentation, as they are generally faster than higher-order tensor-based methods.}

\hy{[EDA helps ML] Unlike existing directed graphs (e.g. financial flow network or social networks), circuits are directed graphs with strong logic reasoning and flow control along the directed edges. EDA tasks serves as a very important real-world application to showcase and validate ML design progress.}

\nan{Not sure whether we should put this: circuit graphs usually have hierarchical structures, involving both local logic reasoning and long-distance reliance.}

\hy{$\bullet$ Question 3. How to position our work? benefits compared with others?}

\hy{1. GPS~\cite{rampavsek2022recipe}: 
\textbf{application: }undirected graph benchmarks (e.g. OGB)
\textbf{method: } GNN + transformer
\textbf{task: graph-level / node-level tasks.} 
\textbf{limitation: } transformer structure is not time/space-efficient in large graphs, and it's not specially designed for directed graphs.
\textbf{comparison: } take GPS as a backbone in low/mid node number tasks.} \pan{We are not to compare the methods therein. We are to compare, from benchmark and insights, what is different from this previous benchmark.}


\hy{2. PyGSD~\cite{he2022pytorch}:
\textbf{application: } social network / financial flow map represented as a single graph. 
\textbf{method: } encoders are mostly spectral methods based on graph filtering
\textbf{task: } node property prediction, link prediction
\textbf{limitation: } not for graph data with various structures, not designed for graph-level tasks.
\textbf{comparison: } take the best in the paper MSGNN~\cite{he2022msgnn} as a baseline.}

\hy{3. HLSYN~\cite{bai2023towards}:
\textbf{application: } HLS prediction task
\textbf{method: } code2vec based methods, pre-trained large transformers, GNNs, 
\textbf{task: } specific graph-level lut/dsp/ff... tasks
\textbf{limitation: } focus on specific tasks}
We may not need to highlight difference between this paper.

\hy{Ours:
\textbf{application: } 5 datasets w/ 13 tasks in EDA domain, formed as directed graphs
\textbf{method: } GNN backbone usage, message passing control, PE design
\textbf{task: } graph-level / node-level}

\hy{$\bullet$ Question 4: contribution}

\hy{\textbf{benchmark: } collect very valuable data (real-world application) to test message passing and PE \pan{do not emphasize PE here. emphasize various and more expressive directed graph encodeer}}

\hy{\textbf{insights and knowledge: }
1. for ML people: [message passing]bi>plain>di, [PE] adding edge-level stable magPE helps [OOD] OOD works on adequate structures or locality node-level tasks. 
2. for EDA people: may try the designing strategy, logic reasoning (bi-directed), long distance control (PE).}

\hy{\textbf{engineering contribution: } a toolbox for directed graph data: module design, auto-ML tuning, training + testing, with data input as required formats.}


1. Many data could be formed as graphs $\rightarrow$ 
undirected graphs (biological network, city map, communication network), 
directed graphs (citation network, knowledge graph, social network and circuit graphs). $\rightarrow$ ML tech fast develop and GNNs are developed to encode or represent graph data:
(1) Designing GNN Encoders for various type of undirected graphs have been well studied [citations of GCN , moleculeGNN, GPS..] \pan{do not spend that much space on undirected graphs.}, (2) recent interest in directed graphs, where no longer symmetric adjacency matrix, instead has further challenges in handling the directed edges[citations of directed methods ~\cite{rossi2023edge, wen2020neural, kollias2022directed, jaume2019edgnn, hussain2022global, geisler2023transformers}]. 
$\rightarrow$ 2 types of directed graphs: (1)For directed networks like citation/social/finance networks \pan{do not need to mention these, or at least they should not be presented here}, where mostly use single graph \pan{single graph is a improfessional point to be argued as a difference}, the graph is dynamic and large, node/edge-level tasks are preferred, encoder designing principles based on spectral theory and graph filtering are well discussed[citations: ~\cite{he2022pytorch} and all related methods], 
(2) circuit graphs could represent another kind of directed graph, with more static, with much stronger logic reasoning, and relatively long-distance flow control, the spectral/filtering principles may no longer be useful. \nan{from the application side, people usually care more about inter-graph generalization.} Though also many wonderful works for circuits [citation: ML for circuit], but they are task-specific designs with the help of expertise knowledge in specific tasks \pan{task-specific design is not a problem...} \nan{maybe we can say: structural information is mostly manually crafted by human experts. This can motivate learning-based more expressive encoders for structural information.}, here we pose an interesting question: Can advanced GNN techs help design encoders for this type of graph that might be able to serve as a general baseline? 

\pan{the above is a so-so starting paragraph. Your paragraph has no EDA significance, purely for ML. Suggested: 1. Why EDA needs ML? 2. EDA data can be represented as directed graphs. 3. What are the properties of these graphs? Why they may be challenging? (logic dependence, local inductive bias, long range dependence, some are large) 4. Do previous benchmarks in graph ML provide insights in the models for these graphs? Therefore, we need a benchmark }


2. To answer the questions, we collect 5 circuit datasets, 13 different circuit tasks, including $4$ steps in \nan{digital} IC design and an analog circuit dataset as valuable real-world directed graph application alternative than social/finance networks to benchmark the designing strategies of GNNs. We investigate the choice of GNN backbones, message passing control (tell which is suitable for strong local logic reasoning), and PE design \pan{more expressive power is what one needs for PE motivation, long-range dependence, only telling long range why transformer is not sufficient to solve the problem?} (tell which is suitable for long-distance dependency) for circuit graphs. 

\pan{We collect xxx datasets. 1. whether they are representative? 2. are they sufficient to cover different applications?  Basically, why do we choose these datasets? 3. Do they introduce sufficient challenges to ML methods? 4. Use these challenges to motivate the methods we are to include. Expressiveness, scalability, stability etc. 5. Due to the need of expressiveness, scalaiblity, stability, this benchmark also works a valuable testbeds for evluation directed graph representation learning methods. }




3. From our experiments we can tell that, for directed graphs such as circuits with strong logic reasoning requirement, bi-weight is the best message passing strategy, stable PE is useful in directed graphs that require some long-distance flow dependency. For OOD generalization, dataset with adequate graph structures or rely on local structures is good, otherwise is still challenging. These insights might  also provide some knowledge to the EDA domain that might be helpful for further encoder design \pan{too weak statements}.

\pan{Key insights we get should echo with the data properties and challenges we mentioned, expressive power, scalability, (note that stability is necessary for ood)}

\pan{We are to first one consider using stable PE in directed graph encoders. Combine transformer with bignn. List all the first trials we have. Mention we finally obtained xxx model has achieved xxx top xxx among xxx, which is expected to become the most important backbone/baseline for EDA directed graph encoders.  }

We also provide a toolbox for obtaining encoders for directed graph data, including auto-ML hyper-parameter tuning, encoder training and testing, where EDA people may formulate their data in the required data form and do an easy hyper-parameter selection -training-testing.

 \pan{Our benchmark is very modular, which accepts new methods, accepts new datasets, easy for plug-in and play.}
\nan{with well-designed interfaces to take new EDA datasets.}

==> arxiv/tables/amp/amp_gain_qvalue.tex <==

\begin{table}[h]
\centering
\begin{tabular}{@{}ccc@{}}
\toprule
method & \multicolumn{2}{c}{gain} \\ \cmidrule(l){2-3} 
 & mse & rmse \\ \midrule
GPS+magEPE(q=0.00) & 0.138±0.041 & 0.369±0.051 \\
GPS+magEPE(q=0.01) & \textbf{0.121±0.007} & \textbf{0.348±0.011} \\
GPS+magEPE(q=0.02) & 0.148±0.046 & 0.382±0.053 \\
GPS+magEPE(q=0.05) & 0.145±0.067 & 0.375±0.074 \\
GPS+magEPE(q=0.07) & 0.138±0.017 & 0.370±0.023 \\
GPS+magEPE(q=0.10) & 0.171±0.059 & 0.408±0.065 \\ \bottomrule
\end{tabular}
\caption{AMP q value.}
\label{tab:amp_gain_qvalue}
\end{table}

==> arxiv/tables/performer/time_id_mse.tex <==

%\begin{table}[h]
\begin{center}
    \resizebox{\textwidth}{!}{\begin{tabular}{cccccccccc}
\hline
task                   & method                  & blabla                & usb\_cdc\_core       & wbqspiflash          & cic\_decimator       & picorv32a             & zipdiv               & usb                  & id avg                \\ \hline
\multirow{8}{*}{hold}  & GINE+magNPE(q=0)        & 0.457±0.079           & 1.736±0.168          & 0.149±0.056          & 0.049±0.023          & 2.303±0.133           & 0.278±0.098          & 0.048±0.018          & 0.717±0.045           \\
                       & GINE+magNPE(q=0.1)      & 1.108±0.712           & 0.155±0.053          & 0.372±0.093          & 0.047±0.016          & 1.804±0.085           & 0.116±0.109          & 0.045±0.008          & 0.521±0.125           \\
                       & GINE+magEPE(q=0)        & 0.163±0.027           & \textbf{0.027±0.009} & 0.033±0.003          & \textbf{0.011±0.006} & \textbf{0.518±0.043}  & 0.012±0.006          & \textbf{0.017±0.003} & \textbf{0.112±0.007}  \\
                       & GINE+magEPE(q=0.1)      & \textbf{0.145±0.010}  & 0.030±0.011          & 0.034±0.018          & 0.113±0.135          & \textbf{0.479±0.073}  & 0.231±0.093          & 0.020±0.010          & 0.150±0.024           \\ \cline{2-10} 
                       & PERFORMER+magNPE(q=0)   & 0.415±0.091           & 1.846±0.170          & 0.204±0.055          & 0.140±0.064          & 2.308±0.084           & 0.413±0.104          & 0.078±0.017          & 0.772±0.036           \\
                       & PERFORMER+magNPE(q=0.1) & 0.334±0.091           & 0.283±0.110          & 0.160±0.049          & 0.105±0.029          & 1.973±0.093           & 0.176±0.104          & 0.051±0.011          & 0.440±0.028           \\
                       & PERFORMER+magEPE(q=0)   & \textbf{0.180±0.020}  & 0.034±0.012          & 0.038±0.003          & 0.017±0.007          & 0.933±0.428           & \textbf{0.020±0.007} & 0.037±0.012          & 0.180±0.062           \\
                       & PERFORMER+magEPE(q=0.1) & 0.162±0.024           & \textbf{0.027±0.007} & \textbf{0.026±0.008} & 0.028±0.023          & 0.886±0.472           & 0.300±0.071          & 0.018±0.005          & 0.207±0.075           \\ \hline
\multirow{8}{*}{setup} & GINE+magNPE(q=0)        & 56.090±3.348          & 4.263±0.847          & 11.020±1.890         & 1.712±0.674          & 32.027±2.138          & 9.328±2.138          & 1.562±0.283          & 16.572±0.880          \\
                       & GINE+magNPE(q=0.1)      & 53.133±11.049         & 3.849±0.427          & 14.508±2.511         & 1.545±0.393          & 29.165±1.697          & 12.165±2.065         & 2.058±0.420          & 16.632±1.869          \\
                       & GINE+magEPE(q=0)        & \textbf{26.166±5.021} & \textbf{2.064±0.662} & \textbf{7.886±3.039} & \textbf{1.720±0.574} & \textbf{34.451±7.187} & \textbf{6.805±4.672} & \textbf{1.528±0.344} & \textbf{11.517±2.081} \\
                       & GINE+magEPE(q=0.1)      & 70.852±54.789         & 5.614±6.407          & 12.512±13.792        & 6.057±13.390         & 39.247±16.729         & 12.607±13.468        & 5.670±5.327          & 21.794±16.003         \\ \cline{2-10} 
                       & PERFORMER+magNPE(q=0)   & 71.180±7.296          & 6.017±0.951          & 19.114±3.978         & 2.786±0.931          & 40.219±2.599          & 21.280±5.284         & 1.974±0.394          & 23.224±2.482          \\
                       & PERFORMER+magNPE(q=0.1) & 76.600±6.188          & 6.559±2.542          & 22.725±1.503         & 15.529±9.577         & 39.556±2.732          & 23.995±3.420         & 4.789±1.457          & 27.107±0.881          \\
                       & PERFORMER+magEPE(q=0)   & 126.117±80.432        & 9.430±7.367          & 27.358±10.385        & 13.462±10.786        & 50.999±8.878          & 25.830±8.329         & 6.231±5.001          & 37.061±12.283         \\
                       & PERFORMER+magEPE(q=0.1) & 99.647±56.437         & 7.066±5.571          & 18.282±10.408        & 6.835±10.700         & 53.188±7.057          & 14.306±4.984         & 3.296±2.664          & 28.946±11.880         \\ \hline
\end{tabular}}
\vspace{-0.3cm}
\captionof{table}{GPS w/ `PERFORMER' v.s. GINE on the TIME dataset on ID data with metric `mse'.}
\label{tab:performer_id_mse}
\end{center}
%\end{table}

==> arxiv/tables/performer/time_id_r2.tex <==
%\begin{table}[h]
\begin{center}
    

\resizebox{\textwidth}{!}{\begin{tabular}{cccccccccc}
\hline
task                   & method                  & blabla                                            & usb\_cdc\_core                           & wbqspiflash                              & cic\_decimator                           & picorv32a                                & zipdiv                                   & usb                                      & id avg                                   \\ \hline
\multirow{8}{*}{hold}  & GINE+magNPE(q=0)        & \multicolumn{1}{l}{0.995±0.000}                   & \multicolumn{1}{l}{0.078±0.089}          & \multicolumn{1}{l}{0.913±0.032}          & \multicolumn{1}{l}{0.967±0.015}          & \multicolumn{1}{l}{0.839±0.009}          & \multicolumn{1}{l}{0.934±0.023}          & \multicolumn{1}{l}{0.954±0.017}          & \multicolumn{1}{l}{0.811±0.012}          \\
                       & GINE+magNPE(q=0.1)      & \multicolumn{1}{l}{0.989±0.006}                   & \multicolumn{1}{l}{0.921±0.026}          & \multicolumn{1}{l}{0.863±0.034}          & \multicolumn{1}{l}{0.946±0.018}          & \multicolumn{1}{l}{0.869±0.006}          & \multicolumn{1}{l}{0.967±0.030}          & \multicolumn{1}{l}{0.934±0.011}          & \multicolumn{1}{l}{0.927±0.012}          \\
                       & GINE+magEPE(q=0)        & \multicolumn{1}{l}{\textbf{0.998±0.000}}          & \multicolumn{1}{l}{\textbf{0.985±0.005}} & \multicolumn{1}{l}{0.980±0.001}          & \multicolumn{1}{l}{\textbf{0.992±0.004}} & \multicolumn{1}{l}{\textbf{0.963±0.003}} & \multicolumn{1}{l}{\textbf{0.996±0.001}} & \multicolumn{1}{l}{\textbf{0.983±0.003}} & \multicolumn{1}{l}{\textbf{0.985±0.001}} \\
                       & GINE+magEPE(q=0.1)      & \multicolumn{1}{l}{\textit{\textbf{0.998±0.000}}} & \multicolumn{1}{l}{0.984±0.005}          & \multicolumn{1}{l}{\textbf{0.987±0.006}} & \multicolumn{1}{l}{0.872±0.151}          & \multicolumn{1}{l}{\textbf{0.965±0.005}} & \multicolumn{1}{l}{0.936±0.025}          & \multicolumn{1}{l}{0.971±0.014}          & \multicolumn{1}{l}{0.959±0.022}          \\ \cline{2-10} 
                       & PERFORMER+magNPE(q=0)   & 0.996±0.000                                       & 0.020±0.090                              & 0.881±0.032                              & 0.907±0.042                              & 0.839±0.005                              & 0.903±0.024                              & 0.925±0.016                              & 0.782±0.014                              \\
                       & PERFORMER+magNPE(q=0.1) & 0.996±0.000                                       & 0.856±0.055                              & 0.941±0.018                              & 0.881±0.033                              & 0.857±0.006                              & 0.951±0.028                              & 0.927±0.016                              & 0.916±0.017                              \\
                       & PERFORMER+magEPE(q=0)   & \textbf{0.998±0.000}                              & 0.981±0.006                              & 0.977±0.002                              & 0.988±0.005                              & 0.934±0.029                              & 0.995±0.001                              & 0.964±0.011                              & 0.977±0.004                              \\
                       & PERFORMER+magEPE(q=0.1) & \textbf{0.998±0.000}                              & \textbf{0.986±0.003}                     & \textbf{0.990±0.003}                     & 0.967±0.026                              & 0.936±0.034                              & 0.917±0.019                              & 0.973±0.007                              & 0.967±0.009                              \\ \hline
\multirow{8}{*}{setup} & GINE+magNPE(q=0)        & 0.139±0.051                                       & 0.205±0.157                              & 0.429±0.097                              & 0.192±0.317                              & 0.231±0.051                              & 0.536±0.106                              & 0.373±0.113                              & 0.301±0.054                              \\
                       & GINE+magNPE(q=0.1)      & 0.256±0.154                                       & 0.213±0.087                              & 0.312±0.119                              & \textbf{0.261±0.188}                     & \textbf{0.224±0.045}                     & 0.387±0.104                              & 0.316±0.139                              & 0.281±0.073                              \\
                       & GINE+magEPE(q=0)        & \textbf{0.598±0.076}                              & \textbf{0.615±0.123}                     & \textbf{0.591±0.157}                     & 0.188±0.270                              & 0.172±0.172                              & \textbf{0.662±0.231}                     & \textbf{0.386±0.138}                     & \textbf{0.459±0.114}                     \\
                       & GINE+magEPE(q=0.1)      & 0.009±0.766                                       & -0.146±1.308                             & 0.407±0.653                              & -1.895±6.399                             & -0.043±0.444                             & 0.364±0.678                              & -0.884±1.769                             & -0.312±1.494                             \\ \cline{2-10} 
                       & PERFORMER+magNPE(q=0)   & -0.091±0.111                                      & -0.121±0.177                             & 0.010±0.205                              & -0.313±0.439                             & 0.034±0.062                              & -0.056±0.262                             & 0.207±0.158                              & -0.047±0.151                             \\
                       & PERFORMER+magNPE(q=0.1) & -0.071±0.086                                      & -0.339±0.519                             & -0.076±0.071                             & -6.422±4.577                             & -0.052±0.072                             & -0.208±0.172                             & -0.591±0.484                             & -1.108±0.654                             \\
                       & PERFORMER+magEPE(q=0)   & -0.933±1.233                                      & -0.757±1.372                             & -0.415±0.537                             & -5.347±5.085                             & -0.224±0.213                             & -0.282±0.413                             & -1.500±2.006                             & -1.351±1.123                             \\
                       & PERFORMER+magEPE(q=0.1) & -0.393±0.789                                      & -0.443±1.137                             & 0.133±0.493                              & -2.267±5.113                             & -0.414±0.187                             & 0.279±0.251                              & -0.095±0.885                             & -0.457±1.148                             \\ \hline
\end{tabular}}
\vspace{-0.3cm}
\captionof{table}{GPS w/ `PERFORMER' v.s. GINE on the TIME dataset on ID data with metric `R2'.}
\label{tab:performer_id_r2}
\end{center}
%\end{table}

==> arxiv/tables/performer/time_ood.tex <==
%\begin{table}[h]
\begin{center}
\resizebox{\textwidth}{!}{\begin{tabular}{cccccc}
\hline
                       &                         & \multicolumn{2}{c}{xtea}                       & \multicolumn{2}{c}{synth\_ram}                                 \\ \cline{3-6} 
                       &                         & mse↓                   & r2↑                   & mse↓                      & r2↑                                \\ \hline
\multirow{8}{*}{hold}  & GINE+magNPE(q=0)        & 7.906±1.090            & -0.245±0.171          & 0.985±0.426               & 0.733±0.115                        \\
                       & GINE+magNPE(q=0.1)      & 6.290±0.964            & 0.008±0.151           & 7.816±7.857               & -1.113±2.124                       \\
                       & GINE+magEPE(q=0)        & 2.185±0.938            & 0.655±0.147           & \textbf{0.790±0.544}      & \textbf{0.786±0.147}               \\
                       & GINE+magEPE(q=0.1)      & 3.911±1.354            & 0.383±0.213           & 2.797±1.947               & 0.243±0.526                        \\ \cline{2-6} 
                       & PERFORMER+magNPE(q=0)   & 7.241±0.520            & -0.140±0.082          & 3.557±0.623               & -0.483±0.365                       \\
                       & PERFORMER+magNPE(q=0.1) & 6.847±0.879            & -0.078±0.138          & 6.704±5.834               & -0.812±1.577                       \\
                       & PERFORMER+magEPE(q=0)   & 2.320±0.774            & 0.634±0.122           & 6.741±4.082               & -0.822±1.103                       \\
                       & PERFORMER+magEPE(q=0.1) & \textbf{1.807±0.612}   & \textbf{0.715±0.096}  & 3.025±2.561               & 0.182±0.692                        \\ \hline
\multirow{8}{*}{setup} & GINE+magNPE(q=0)        & 116.055±40.827         & -2.911±1.376          & 590.409±136.786           & -1140.049±264.359                  \\
                       & GINE+magNPE(q=0.1)      & 101.987±35.767         & -2.437±1.205          & 515.079±104.084           & -994.463±201.157                   \\
                       & GINE+magEPE(q=0)        & 87.633±21.131          & -1.953±0.712          & 865.468±687.014           & -1671.640±1327.753                 \\
                       & GINE+magEPE(q=0.1)      & \textbf{61.823±18.013} & \textbf{-1.083±0.607} & 790.163±227.590           & -1526.102±439.851                  \\ \cline{2-6} 
                       & PERFORMER+magNPE(q=0)   & 124.375±114.416        & -3.191±3.856          & 82.559±46.321             & -158.557±89.522                    \\
                       & PERFORMER+magNPE(q=0.1) & 412.567±168.322        & -12.905±5.673         & \textbf{72.483±66.727}    & \textit{\textbf{-139.085±128.960}} \\
                       & PERFORMER+magEPE(q=0)   & \textbf{94.024±32.056} & \textbf{-2.169±1.080} & 552.117±635.837           & -1066.046±1228.845                 \\
                       & PERFORMER+magEPE(q=0.1) & 81.162±23.368          & -1.735±0.787          & \textbf{1219.394±511.474} & \textbf{-2355.653±988.497}         \\ \hline
\end{tabular}}
\vspace{-0.3cm}
\captionof{table}{GPS w/ `PERFORMER' v.s. GINE on the TIME dataset on OOD data.}
\label{tab:performer_ood}
\end{center}
%\end{table}

==> arxiv/tables/q_value.tex <==
\begin{table}[h]
\centering
\begin{tabular}{ccc}
\hline
method & \multicolumn{2}{c}{AMP gain (ID)}  \\ \cline{2-3} 
 & mse & rmse  \\ \hline
GPS+magEPE(q=0.00) & 0.138±0.041 & 0.369±0.051   \\
GPS+magEPE(q=0.01) & \textbf{0.121±0.007} & \textbf{0.348±0.011}   \\
GPS+magEPE(q=0.02) & 0.148±0.046 & 0.382±0.053   \\
GPS+magEPE(q=0.05) & 0.145±0.067 & 0.375±0.074   \\
GPS+magEPE(q=0.07) & 0.138±0.017 & 0.370±0.023   \\
GPS+magEPE(q=0.10) & 0.171±0.059 & 0.408±0.065   \\ \hline
\end{tabular}
\caption{Performance of GPS w.r.t. different $q$ value selections on the AMP (ID) dataset.}
\label{tab:amp_gain_qvalue}
\end{table}

==> arxiv/tables/summary/backbone_mp.tex <==
\begin{wraptable}{l}{0.5\textwidth} 
    \centering
    \begin{minipage}{\linewidth}
        \centering
        \begin{tabular}{ccc}
\hline
 & spectral/spatial & \begin{tabular}[c]{@{}c@{}}layer-wise\\ complexity\end{tabular} \\ \hline
GCN~\cite{kipf2016semi} & spectral & $O(|E|)$ \\
GAT~\cite{velivckovic2017graph} & spatial & $O(|E|)$ \\
GIN~\cite{xu2018powerful} & spatial & $O(|E|)$ \\
GPS-T~\cite{rampavsek2022recipe} & spatial+transformer & $O(|V|^2 + |E|)$ \\
GPS-P~\cite{choromanski2020rethinking} & spatial+transformer & $O(|V|+|E|)$ \\ \hline
MagNet~\cite{zhang2021magnet} & spectral & $O(|E|)$ \\
DGCN~\cite{tong2020directed} & spectral & $O(|E|)$ \\
DiGCN~\cite{tong2020digraph} & spectral & $O(|E|)$ \\ \hline
\end{tabular}
        \caption{Methods.}
    \end{minipage}
    \vspace{0.5cm} % 插入垂直间距
    \begin{minipage}{\linewidth}
        \centering
        \begin{tabular}{@{}cc@{}}
\toprule
message passing   & description \\ \midrule
`plane' (-)       & $\overset{\rightarrow}{\theta_{\phi}} = \overset{\leftarrow}{\theta_{\phi}} \neq \mathbf{0}$            \\
`directed' (DI)   & $\overset{\rightarrow}{\theta_{\phi}} \neq \mathbf{0},  \overset{\leftarrow}{\theta_{\phi}} = \mathbf{0}$            \\
`bidirected' (BI) & $\overset{\rightarrow}{\theta_{\phi}} \neq \mathbf{0},  \overset{\leftarrow}{\theta_{\phi}} \neq \mathbf{0}, \overset{\rightarrow}{\theta_{\phi}} \neq \overset{\leftarrow}{\theta_{\phi}}$            \\ \bottomrule
\end{tabular}
        \caption{Message passing stratgies.}
    \end{minipage}
\end{wraptable}

==> arxiv/tables/summary/backbone_selection_id.tex <==
\begin{table}[h]
\vspace{-0.4cm}
\centering
\renewcommand{\arraystretch}{0.8}
\resizebox{0.9\textwidth}{!}{\begin{tabular}{@{}ccccccccccccccc@{}}
\toprule
\multicolumn{2}{c}{} & \multicolumn{3}{c}{HLS} & \multicolumn{3}{c}{AMP} & \multicolumn{2}{c}{SR} & \multicolumn{2}{c}{TIME} & \multicolumn{3}{c}{CG} \\ \cmidrule(l){3-15} 
\multicolumn{2}{c}{\multirow{-2}{*}{\textbf{In-Distribution}}} & DSP & LUT & CP & gain & PM & BW & share & root & hold & setup & CPU & GPU630 & GPU640 \\ \midrule 
 & DGCN & 15.0 & 15.0 & 15.0 & 14.0 & 8.0 & 15.0 & 10.0 & 9.0 & 15.0 & 5.5 & 13.0 & 15.0 & 14.0 \\
 & DiGCN & 12.0 & 14.0 & 13.0 & 12.0 & 9.0 & 14.0 & 8.5 & 7.8 & 13.5 & 15.0 & 14.0 & 14.0 & 15.0 \\
 & MagNet & 7.0 & 7.0 & 10.5 & 8.0 & 11.0 & 8.0 & \cellcolor{1}1.8 & \cellcolor{1}2.0 & 11.0 & 11.5 & \cellcolor{1}1.3 & \cellcolor{1}1.3 & 4.7 \\ 
 & GCN & 14.0 & 12.0 & 14.0 & 15.0 & 13.0 & 12.0 & 13.3 & 13.5 & 9.5 & 14.0 & 15.0 & 12.3 & 11.7 \\
 & DI-GCN & 13.5 & 13.0 & 12.0 & 11.0 & \cellcolor{3}3.0 & 13.0 & 15.0 & 15.0 & 11.0 & 13.0 & 11.0 & 11.3 & 12.0 \\
\multirow{-6}{*}{Spectral} & BI-GCN & 11.0 & 10.5 & 9.0 & 5.0 & 14.0 & 6.0 & 5.5 & 5.3 & 5.0 & 9.0 & 12.3 & 12.3 & 12.3 \\ \midrule
 & GIN & 6.0 & 5.5 & 8.0 & 7.0 & 6.0 & 10.0 & 10.0 & 11.0 & \cellcolor{1}1.0 & \cellcolor{3}3.0 & 5.0 & \cellcolor{3}3.3 & 8.3 \\
 & DI-GIN & \cellcolor{2}2.5 & 4.0 & 6.5 & 9.0 & 10.0 & 7.0 & 6.5 & \cellcolor{2}4.8 & \cellcolor{3}3.0 & \cellcolor{2}2.0 & 5.7 & 8.0 & \cellcolor{3}3.3 \\
 & BI-GIN & \cellcolor{1}1.0 & \cellcolor{1}1.0 & 5.0 & \cellcolor{3}3.0 & 4.0 & \cellcolor{3}3.0 & \cellcolor{2}2.8 & \cellcolor{2}4.8 & \cellcolor{2}2.0 & \cellcolor{1}1.0 & \cellcolor{2}2.3 & 4.7 & \cellcolor{1}1.0 \\
 & GAT & 8.5 & 9.0 & 6.5 & 6.0 & 15.0 & 5.0 & 13.8 & 13.5 & 10.5 & 11.5 & 9.0 & 9.0 & 8.7 \\
 & DI-GAT & 10.0 & 10.5 & 10.5 & 10.0 & 12.0 & 9.0 & 11.8 & 10.0 & 13.5 & 10.0 & 10.0 & 10.0 & 10.0 \\
\multirow{-6}{*}{Spatial} & BI-GAT & 9.0 & 8.0 & \cellcolor{1}1.0 & 4.0 & \cellcolor{2}2.0 & 11.0 & \cellcolor{3}4.0 & 6.3 & 6.5 & 7.5 & 8.0 & 5.3 & 7.0 \\ \midrule
 & GPS-T & 4.0 & \cellcolor{3}3.0 & \cellcolor{3}2.5 & 13.0 & 7.0 & \cellcolor{2}2.0 & - - & - - & - - & - - & - - & - - & - - \\
 & DI-GPS-T & 5.0 & 5.5 & 4.0 & \cellcolor{1}1.0 & 5.0 & \cellcolor{1}1.0 & - - & - - & - - & - - & - - & - - & - - \\
 & BI-GPS-T & \cellcolor{3}3.0 & \cellcolor{2}2.0 & \cellcolor{2}2.0 & \cellcolor{1}1.0 & \cellcolor{1}1.0 & 4.0 & - - & - - & - - & - - & - - & - - & - - \\
 & GPS-P & - - & - - & - - & - - & - - & - - & 5.5 & 12.0 & 6.5 & 4.0 & 6.3 & \cellcolor{2}2.0 & 5.3 \\
 & DI-GPS-P & - - & - - & - - & - - & - - & - - & 6.5 & \cellcolor{2}4.8 & 4.0 & 7.5 & \cellcolor{3}2.7 & 5.7 & \cellcolor{1}3.0 \\
\multirow{-6}{*}{Transformer} & BI-GPS-P & - - & - - & - - & - - & - - & - - & 7.8 & 7.5 & 8.0 & 5.5 & 4.7 & 6.0 & 4.3 \\ \bottomrule
 \end{tabular}}
\caption{Average ranking ($\downarrow$) of methods across datasets/tasks/metrics on in-distribution data.}
\label{tab:exp_gnn_backbone_selection_id}
\vspace{-0.5cm}
\end{table}

==> arxiv/tables/summary/backbone_slection_ood.tex <==
\begin{table}[h]
\vspace{-0.4cm}
\centering
\renewcommand{\arraystretch}{0.8}
\resizebox{0.9\textwidth}{!}{\begin{tabular}{@{}ccccccccccccccc@{}}
\toprule
\multicolumn{2}{c}{} & \multicolumn{3}{c}{HLS} & \multicolumn{3}{c}{AMP} & \multicolumn{2}{c}{SR} & \multicolumn{2}{c}{TIME} & \multicolumn{3}{c}{CG} \\ \cmidrule(l){3-15} 
\multicolumn{2}{c}{\multirow{-2}{*}{\textbf{Out-of-Distribution}}} & DSP & LUT & CP & gain & PM & BW & share & root & hold & setup & CPU & GPU630 & GPU640 \\ \midrule
 & DGCN & 15.0 & 14.0 & 15.0 & 14.0 & \cellcolor{3}3.0 & 15.0 & 7.5 & 5.0 & 15.0 & 7.0 & 13.3 & 11.7 & 11.2 \\
 & DiGCN & 12.5 & 15.0 & 14.0 & 9.0 & 4.0 & 14.0 & 9.0 & 5.0 & 13.5 & 14.0 & 13.2 & 13.2 & 13.3 \\
 & MagNet & 7.0 & 7.0 & 10.5 & \cellcolor{3}3.0 & 12.0 & 8.0 & \cellcolor{3}3.5 & 8.8 & 9.0 & 7.0 & \cellcolor{3}4.2 & 8.2 & 7.3 \\ 
 & GCN & 12.5 & 10.0 & 12.0 & 14.5 & 114.0 & 11.0 & 14.8 & 14.5 & 7.5 & 10.5 & 12.7 & 12.7 & 11.5 \\
 & DI-GCN & 14.0 & 11.0 & 13.0 & 12.0 & 7.0 & 13.0 & 13.5 & 11.8 & 10.0 & 8.0 & 11.2 & 11.5 & 12.2 \\
\multirow{-6}{*}{Spectral} & BI-GCN & 11.0 & 12.5 & 8.0 & \cellcolor{2}2.0 & 13.0 & 5.0 & \cellcolor{2}2.3 & \cellcolor{3}4.8 & \cellcolor{2}3.0 & \cellcolor{2}6.5 & 13.2 & 11.3 & 12.5 \\ \midrule
 & GIN & 6.0 & \cellcolor{3}3.5 & 5.0 & 8.0 & 10.0 & 7.0 & 9.0 & 7.3 & \cellcolor{2}3.0 & 8.5 & 5.2 & \cellcolor{1}4.2 & 4.8 \\
 & DI-GIN & \cellcolor{1}2.0 & \cellcolor{2}2.5 & 7.0 & 10.0 & 5.0 & 12.0 & 6.3 & 9.0 & 6.5 & 7.0 & \cellcolor{2}3.5 & 5.7 & \cellcolor{2}4.2 \\
 & BI-GIN & 4.5 & \cellcolor{1}1.0 & \cellcolor{2}3.0 & \cellcolor{3}4.0 & 9.0 & 3.0 & \cellcolor{1}1.5 & \cellcolor{1}2.0 & \cellcolor{1}1.0 & 7.5 & \cellcolor{1}2.3 & \cellcolor{3}4.5 & \cellcolor{1}4.0 \\
 & GAT & 9.0 & 9.0 & 5.5 & 7.0 & 15.0 & 6.0 & 12.3 & 10.5 & 10.5 & \cellcolor{1}5.5 & 7.7 & 5.7 & 6.2 \\
 & DI-GAT & 10.0 & 12.5 & 11.0 & 11.0 & 6.0 & 10.0 & 11.3 & 10.0 & 13.5 & 8.5 & 6.2 & 5.7 & 7.3 \\
\multirow{-6}{*}{Spatial} & BI-GAT & 8.0 & 8.0 & \cellcolor{1}1.5 & \cellcolor{1}1.0 & \cellcolor{2}2.0 & 9.0 & 9.8 & 8.5 & 4.5 & \cellcolor{2}6.5 & 6.2 & 10.7 & 10.5 \\ \midrule
 & GPS-T & 5.0 & 6.0 & 9.5 & 13.0 & 8.0 & \cellcolor{1}1.0 & - - & - - & - - & - - & - - & - - & - - \\
 & DI-GPS-T & \cellcolor{3}3.0 & 5.0 & \cellcolor{1}1.5 & 5.0 & 11.0 & \cellcolor{2}2.0 & - - & - - & - - & - - & - - & - - & - - \\
 & BI-GPS-T & \cellcolor{2}2.5 & \cellcolor{3}3.5 & \cellcolor{3}4.5 & 6.0 & \cellcolor{1}1.0 & 4.0 & - - & - - & - - & - - & - - & - - & - - \\
 & GPS-P & - - & - - & - - & - - & - - & - - & 7.8 & 11.3 & 8.0 & 7.5 & 6.2 & \cellcolor{1}4.2 & 6.2 \\
 & DI-GPS-P & - - & - - & - - & - - & - - & - - & 5.8 & 7.5 & 7.5 & 8.0 & 7.5 & 7.0 & 5.8 \\
\multirow{-6}{*}{Transformer} & BI-GPS-P & - - & - - & - - & - - & - - & - - & 6.8 & \cellcolor{2}4.3 & 7.5 & 8.0 & 8.5 & 5.2 & \cellcolor{2}4.2 \\ \bottomrule
\end{tabular}}
\caption{Average ranking ($\downarrow$) of methods across datasets/tasks/metrics on out-of-distribution data.}
\label{tab:exp_gnn_backbone_selection_ood}
\vspace{-0.5cm}
\end{table}

==> arxiv/tables/summary/bidi.tex <==

\begin{wraptable}{r}{0.44\textwidth}
\vspace{-0.35cm}
\small
\renewcommand{\arraystretch}{0.85}
\centering
\begin{tabular}{@{}ccc@{}}
\toprule
 & ID ranking $\downarrow$ & OOD ranking $\downarrow$ \\ \midrule
GCN & 2.778 & 2.350 \\
DIGCN & 2.383 & 2.233 \\
BIGCN & \textbf{1.439} & \textbf{1.417} \\ \midrule
GIN(E) & 2.639 & 2.433 \\
DIGIN(E) & 2.694 & 2.244 \\
BIGIN(E) & \textbf{1.267} & \textbf{1.378} \\ \midrule
GAT & 2.222 & 2.044 \\
DIGAT & 2.922 & 2.483 \\
BIGAT & \textbf{1.456} & \textbf{1.483} \\ \bottomrule
\end{tabular}
\vspace{-0.2cm}
\caption{Average rankings of GCN, GIN(E), GAT with (-), (DI), and (BI) strategy. \pan{remove this one}}
\vspace{-0.4cm}
\label{tab:bidi}
\end{wraptable}

==> arxiv/tables/summary/id_ood.tex <==
\begin{wraptable}{r}{0.45\textwidth}
\vspace{-0.3cm}
\renewcommand{\arraystretch}{0.6}
\resizebox{0.45 \textwidth}{!}{\begin{tabular}{@{}ccccc@{}}
\toprule
 & \multicolumn{2}{c}{in-distribution} & \multicolumn{2}{c}{out-of-distribution} \\ \midrule
 & \#top1 $\uparrow$ & \#top3$\uparrow$ & \#top1$\uparrow$ & \#top3$\uparrow$ \\ \midrule
GCN & 0.00 & 0.00 & 0.00 & 0.00 \\
DIGCN & 0.00 & 0.33 & 0.00 & 0.00 \\
BIGCN & 0.13 & 0.38 & 0.13 & 1.08 \\
GINE & 0.00 & 0.83 & 0.35 & 0.51 \\
DIGINE & 0.25 & 0.86 & 0.17 & 0.81 \\
BIGINE & 0.69 & 2.72 & 0.25 & 1.65 \\
GAT & 0.00 & 0.00 & 0.31 & 0.69 \\
DIGAT & 0.00 & 0.00 & 0.11 & 0.47 \\
BIGAT & 0.33 & 1.00 & 0.67 & 0.67 \\
MSGNN & 1.22 & 1.56 & 0.39 & 0.83 \\ \midrule
GINE+EPE(q=0) & 0.50 & 1.64 & 0.13 & 0.49 \\
GINE+EPE(q=0.1) & 0.25 & 0.99 & 0.18 & 1.29 \\
BIGINE+EPE(q=0) & \textbf{1.42} & \textbf{3.31} & \textbf{1.25} & \textbf{3.18} \\
BIGINE+EPE(q=0.1) & 1.13 & 2.50 & 1.22 & 2.43 \\ \bottomrule
\end{tabular}}
\vspace{-0.3cm}
\caption{Composite scores across all datasets. \pan{perhaps not needed}}
\vspace{-0.5cm}
\label{tab:id_ood}
\end{wraptable}

==> arxiv/tables/summary/ne_id.tex <==

\begin{table}[]
\centering
\resizebox{0.9\textwidth}{!}{\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
\multirow{2}{*}{In-Distribution} & \multicolumn{3}{c}{HLS} & \multicolumn{3}{c}{AMP} & \multicolumn{2}{c}{SR} & \multicolumn{2}{c}{TIME} & \multicolumn{3}{c}{CG} \\ \cmidrule(l){2-14} 
 & DSP & LUT & CP & gain & PM & BW & share & root & hold & setup & CPU & GPU630 & GPU640 \\ \midrule
MagNet & 14.5 & 11.0 & 14.5 & 12.0 & 15.0 & 12.0 & \textbf{2.3} & \textbf{2.5} & 13.0 & 13.0 & 2.3 & \textbf{1.7} & 6.7 \\ \midrule
BI-GIN(E) & 9.0 & 2.0 & 9.0 & 6.0 & 6.0 & 6.0 & 4.8 & 6.8 & 2.5 & 2.0 & 6.0 & 3.3 & 6.0 \\
BI-GIN(E)+NPE & 5.0 & 4.0 & 5.0 & 5.0 & 13.0 & 5.0 & 3.0 & 6.8 & 5.5 & 5.0 & 8.3 & 5.0 & 5.3 \\
BI-GIN(E)+EPE & 5.0 & \textbf{1.0} & 5.0 & 9.0 & 10.0 & \textbf{3.0} & 4.0 & 6.8 & \textbf{2.0} & \textbf{1.0} & \textbf{1.0} & 6.7 & \textbf{1.7} \\ \midrule
BI-GPS-T+NPE & 4.5 & 5.5 & 4.5 & 2.0 & 2.0 & 7.0 & - - & - - & - - & - - & - - & - - & - - \\
BI-GPS-T+EPE & \textbf{2.5} & 3.0 & \textbf{2.0} & \textbf{1.0} & \textbf{1.0} & 4.0 & - - & - - & - - & - - & - - & - - & - - \\ \bottomrule
\end{tabular}}
\caption{Comparison of methods on ID data involving NPE and EPE.}
\vspace{-0.5cm}
\label{tab:ne_id}
\end{table}

==> arxiv/tables/summary/ne_ood.tex <==
\begin{table}[]
\centering
\resizebox{0.9\textwidth}{!}{\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
\multirow{2}{*}{In-Distribution} & \multicolumn{3}{c}{HLS} & \multicolumn{3}{c}{AMP} & \multicolumn{2}{c}{SR} & \multicolumn{2}{c}{TIME} & \multicolumn{3}{c}{CG} \\ \cmidrule(l){2-14} 
 & DSP & LUT & CP & gain & PM & BW & share & root & hold & setup & CPU & GPU630 & GPU640 \\ \midrule
MagNet & 11.0 & 11.0 & 14.5 & \textbf{3.0} & 16.0 & 12.0 & 5.5 & 10.8 & 11.0 & 16.0 & 5.2 & 9.5 & 8.3 \\ \midrule
BI-GIN(E) & 7.5 & 3.5 & 6.0 & 4.0 & 13.0 & 5.0 & 3.0 & \textbf{3.0} & 2.5 & \textbf{7.5} & 4.7 & 5.8 & 4.8 \\
BI-GIN(E)+NPE & 9.0 & 4.0 & \textbf{1.5} & 7.0 & 8.0 & 7.0 & 2.8 & 3.5 & 5.5 & 12.5 & 6.0 & \textbf{4.5} & 6.0 \\
BI-GIN(E)+EPE & 7.0 & \textbf{1.0} & 2.5 & 6.0 & 6.0 & 4.0 & \textbf{1.5} & \textbf{3.0} & \textbf{1.0} & \textbf{7.5} & \textbf{3.8} & 5.5 & \textbf{4.7} \\ \midrule
BI-GPS-T+NPE & 4.0 & 7.0 & 8.0 & 9.0 & 2.0 & 6.5 & - - & - - & - - & - - & - - & - - & - - \\
BI-GPS-T+EPE & \textbf{1.5} & 1.5 & 3.5 & 5.5 & \textbf{1.0} & \textbf{1.0} & - - & - - & - - & - - & - - & - - & - - \\ \bottomrule
\end{tabular}}
\caption{Comparison of methods on OOD data involving NPE and EPE.}
\label{tab:ne_ood}
\end{table}

==> arxiv/tables/time/time_hold_ood.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}
\begin{tabular}{@{}ccccc@{}}
\toprule
method & \multicolumn{2}{c}{xtea} & \multicolumn{2}{c}{synth\_ram} \\ \cmidrule(l){2-5} 
 & mse↓ & r2↑ & mse↓ & r2↑ \\ \midrule
GCN & 6.745±0.853 & -0.062±0.134 & 7.511±1.387 & -1.030±0.375 \\
DIGCN & 7.010±0.592 & -0.104±0.093 & 9.764±2.355 & -1.640±0.636 \\
BIGCN & 5.675±0.784 & 0.105±0.123 & 2.446±0.255 & 0.338±0.069 \\
GINE & 4.446±1.623 & 0.299±0.255 & 2.482±1.650 & 0.328±0.446 \\
DIGINE & 3.075±0.887 & 0.515±0.139 & 9.545±4.222 &  \\
BIGINE & 2.116±0.486 & 0.666±0.076 & 1.314±1.197 & 0.644±0.323 \\
GAT & 7.446±1.012 & -0.173±0.159 & 7.741±1.932 & -1.093±0.522 \\
DIGAT & 10.106±0.961 & -0.592±0.151 & 11.260±1.237 & -2.044±0.334 \\
BIGAT & 5.699±1.155 & 0.101±0.181 & 2.683±0.927 & 0.274±0.250 \\
MSGNN & 8.757±1.044 & -0.379±0.164 & 5.321±1.637 & -0.439±0.442 \\ \midrule
GINE+magEPE(q=0) & 2.185±0.938 & 0.655±0.147 & 0.790±0.544 & 0.786±0.147 \\
GINE+magEPE(q=0.1) & 3.911±1.354 & 0.383±0.213 & 2.797±1.947 & 0.243±0.526 \\
BIGINE+magEPE(q=0) & \textbf{1.888±0.761} & \textbf{0.702±0.120} & 0.746±0.274 & 0.798±0.074 \\
BIGINE+magEPE(q=0.1) & 2.074±0.474 & 0.673±0.074 & \textbf{0.617±0.906} & \textbf{0.832±0.245} \\ \midrule
Time-inspired GNN & -- & 0.9135 & -- & 0.8656 \\ \bottomrule
\end{tabular}
\caption{The OOD performance on time hold.}
\label{tab:time_hold_ood}
\end{table}

==> arxiv/tables/time/time_setup_ood.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}
\begin{tabular}{@{}ccccc@{}}
\toprule
method               & \multicolumn{2}{c}{xtea}                       & \multicolumn{2}{c}{synth\_ram}                     \\ \midrule
                     & mse                    & r2                    & mse                     & r2                       \\
GCN                  & 117.599±4.681          & -2.963±0.157          & 509.769±16.052          & -984.202±31.023          \\
DIGCN                & 116.332±16.048         & -2.920±0.540          & 418.819±24.262          & -808.427±46.890          \\
BIGCN                & 100.915±4.158          & -2.401±0.140          & 371.644±10.433          & -717.255±20.164          \\
GINE                 & 62.927±28.904          & -1.120±0.974          & 1341.500±430.261        & -2591.639±831.541        \\
DIGINE               & 61.694±6.981           & -1.079±0.235          & 612.807±101.175         & -1183.337±195.535        \\
BIGINE               & 83.775±17.953          & -1.823±0.605          & 498.357±239.343         & -962.146±462.565         \\
GAT                  & 96.486±7.970           & -2.251±0.268          & \textbf{347.589±30.441} & \textbf{-670.765±58.833} \\
DIGAT                & 122.242±11.986         & -3.120±0.403          & 375.266±18.144          & -724.255±35.066          \\
BIGAT                & 78.499±6.022           & -1.645±0.202          & 463.886±29.786          & -895.527±57.565          \\
MSGNN                & 93.389±2.734           & -2.147±0.092          & 425.460±18.451          & -821.263±35.659          \\ \midrule
GINE+magEPE(q=0)     & 87.633±21.131          & -1.953±0.712          & 865.468±687.014         & -1671.640±1327.753       \\
GINE+magEPE(q=0.1)   & 61.823±18.013          & -1.083±0.607          & 790.163±227.590         & -1526.102±439.851        \\
BIGINE+magEPE(q=0)   & \textbf{43.225±13.056} & \textbf{-0.456±0.440} & 881.450±197.187         & -1702.527±381.091        \\
BIGINE+magEPE(q=0.1) & 59.401±13.573          & -1.002±0.457          & 619.030±136.176         & -1195.363±263.179        \\ \bottomrule
\end{tabular}
\caption{Time setup ood.}
\label{tab:time_setup_ood}
\end{table}

==> mymath.tex <==
\newcommand{\defeq}{\stackrel{\tiny\mathrm{def}}{=}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\thalf}{\tfrac{1}{2}}


\newcommand{\iid}{\stackrel{\tiny\mathrm{iid}}{\sim}}
\newcommand{\E}{\operatorname{\mathsf E}}
%\newcommand{\K}{\operatorname{\mathsf K}}
\newcommand{\Var}{\operatorname{\mathsf Var}}
\renewcommand{\H}{\operatorname{\mathsf H}}
\newcommand{\I}{\operatorname{\mathsf I}}
\newcommand{\D}{\operatorname{\mathsf D}}
\newcommand{\Cov}{\operatorname{\mathsf Cov}}
\newcommand{\FIM}{\operatorname{\mathcal{F}}}


\newcommand{\R}{\operatorname{\mathbb R}}
\newcommand{\Z}{\operatorname{\mathbb Z}}
\newcommand{\X}{\operatorname{\mathcal X}}
\newcommand{\Y}{\operatorname{\mathcal Y}}


\newcommand{\MVN}{\operatorname{MVN}}
\newcommand{\Normal}{\operatorname{Normal}}
\newcommand{\Beta}{\operatorname{Beta}}
\newcommand{\Bernoulli}{\operatorname{Bernoulli}}
\newcommand{\Categorical}{\operatorname{Categorical}}
\newcommand{\Shuffle}{\operatorname{Shuffle}}


\newcommand{\sign}{\operatorname{sign}}
\newcommand{\logit}{\operatorname{logit}}
\newcommand{\expit}{\operatorname{expit}}
\newcommand{\softmax}{\operatorname{softmax}}
\newcommand{\softplus}{\operatorname{softplus}}
\newcommand{\logsumexp}{\operatorname{logsumexp}}


\newcommand{\tee}{\mathsf{\tiny T}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\trace}{\operatorname{trace}}
\newcommand{\chol}{\operatorname{chol}}
\newcommand{\zeros}{\operatorname{\mathbb{0}}}
\newcommand{\ones}{\operatorname{\mathbb{1}}}
\newcommand{\eye}{\operatorname{I}}


\newcommand{\Encoder}{\operatorname{Encoder}}
\newcommand{\Decoder}{\operatorname{Decoder}}
\newcommand{\MLP}{\operatorname{MLP}}
\newcommand{\ResNet}{\operatorname{ResNet}}
\newcommand{\Augment}{\operatorname{Augment}}


\renewcommand{\dot}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\abs}[1]{\left| #1 \right|}
%\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\newcommand{\ceil}[1]{\left\lceil #1 \rceil|}
\newcommand{\floor}[1]{\left\lfloor #1 \rfloor|}


\newcommand{\domain}{\operatorname{domain}}
\newcommand{\range}{\operatorname{range}}
\newcommand{\ndims}{\operatorname{ndims}}
\newcommand{\shape}{\operatorname{shape}}
\newcommand{\size}{\operatorname{size}}
\newcommand{\len}{\operatorname{len}}
\newcommand{\indexes}{\operatorname{indexes}}



%\theoremstyle{plain}            % use "default" font
\newtheorem{thm}{Theorem}[section]
\newtheorem{lma}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{clm}[thm]{Claim}

%\theoremstyle{definition}       % use "definition-style" font for the rest
\newtheorem{defn}[thm]{Definition}
\newtheorem{examp}[thm]{Example}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{rmk}[thm]{Remark}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}
